Accurate Prediction and Uncertainty Estimation using Decoupled Prediction Interval Networks

We propose a network architecture capable of reliably estimating uncertainty of regression based predictions without sacrificing accuracy. The current state-of-the-art uncertainty algorithms either fall short of achieving prediction accuracy comparable to the mean square error optimization or underestimate the variance of network predictions. We propose a decoupled network architecture that is capable of accomplishing both at the same time. We achieve this by breaking down the learning of prediction and prediction interval (PI) estimations into a two-stage training process. We use a custom loss function for learning a PI range around optimized mean estimation with a desired coverage of a proportion of the target labels within the PI range. We compare the proposed method with current state-of-the-art uncertainty quantification algorithms on synthetic datasets and UCI benchmarks, reducing the error in the predictions by 23 to 34% while maintaining 95% Prediction Interval Coverage Probability (PICP) for 7 out of 9 UCI benchmark datasets. We also examine the quality of our predictive uncertainty by evaluating on Active Learning and demonstrating 17 to 36% error reduction on UCI benchmarks.

==> active/table.tex <==
 \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{RMSE}}}}& MC-Dr & 3.31 $\pm$  0.48 & 6.28 $\pm$  0.33 & 2.02 $\pm$  0.17 & 0.11 $\pm$  0.00 & 0.01 $\pm$  0.00 & 4.20 $\pm$  0.06 & 0.63 $\pm$  0.02 & 1.96 $\pm$  0.31 & 4.63 $\pm$  0.03\\ 
& DeepEns & 3.38 $\pm$  0.63 & 6.12 $\pm$  0.40 & 2.36 $\pm$  0.15 & 0.11 $\pm$  0.01 & 0.01 $\pm$  0.00 & 4.05 $\pm$  0.04 & 0.64 $\pm$  0.03 & 1.11 $\pm$  0.30 & 4.67 $\pm$  0.04\\ 
& Split-Train & 4.33 $\pm$  1.04 & 9.05 $\pm$  1.95 & 1.40 $\pm$  0.24 & 0.18 $\pm$  0.03 & 0.01 $\pm$  0.01 & 4.66 $\pm$  0.53 & 0.88 $\pm$  0.20 & 1.60 $\pm$  0.41 & 6.52 $\pm$  1.69\\ 
& DPIN & 3.23 $\pm$  0.41 & 5.50 $\pm$  0.17 & 0.64 $\pm$  0.07 & 0.08 $\pm$  0.00 & 0.00 $\pm$  0.00 & 4.03 $\pm$  0.05 & 0.66 $\pm$  0.03 & 0.82 $\pm$  0.22 & 4.52 $\pm$  0.03\\ 
\hline\hline \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\texttt{LL}}}}& MC-Dr & 3.30 $\pm$  0.49 & 3.90 $\pm$  0.24 & 2.57 $\pm$  0.24 & -0.60 $\pm$  0.07 & -2.74 $\pm$  0.18 & 4.19 $\pm$  0.06 & 6.62 $\pm$  0.97 & 3.42 $\pm$  0.58 & 11.12 $\pm$  0.66\\ 
& DeepEns & -3.26 $\pm$  0.66 & -3.49 $\pm$  0.30 & -1.57 $\pm$  0.16 & 1.01 $\pm$  0.04 & 3.72 $\pm$  0.05 & -2.80 $\pm$  0.01 & -1.27 $\pm$  0.17 & -0.86 $\pm$  0.06 & -2.86 $\pm$  0.01\\ 
& Split-Train & -370.45 $\pm$  6.79 & -880.32 $\pm$  15.71 & -553.63 $\pm$  13.99 & -160.72 $\pm$  167.50 & 6484.77 $\pm$  931.98 & -8028.25 $\pm$  168.76 & -466.90 $\pm$  57.98 & -247.01 $\pm$  6.00 & -31753.60 $\pm$  1565.18\\ 
& DPIN & -2.54 $\pm$  0.10 & -3.10 $\pm$  0.02 & -1.51 $\pm$  0.06 & 1.02 $\pm$  0.02 & 3.95 $\pm$  0.04 & -2.82 $\pm$  0.01 & -1.01 $\pm$  0.05 & -1.73 $\pm$  0.07 & -2.90 $\pm$  0.01\\ 
\hline\hline

==> exper/archive.tex <==

\begin{table}[h!]
\bgroup
\def\arraystretch{1.2}
\setlength{\tabcolsep}{3pt}
    \centering
    
    \begin{tabular}{c c c c c c c c c }
    \hline
     & \multicolumn{4}{c}{RMSE} & \multicolumn{4}{c}{PICP}\\
     & DeepEns & MC-Dr & Split-train & DVN  & DeepEns &  MC-Dr & Split-train &DVN\\
     \hline
    Boston & 3.38 $\pm$0.26 & 3.13 $\pm$1.02 & 0.26 $\pm$3.13 &3.06 $\pm$1.08 & 2.87 $\pm$0.68 & 0.26 $\pm$3.13 & 3.06 $\pm$1.08 &3.06 $\pm$1.08 \\
    Concrete &5.76 $\pm$0.10 &5.45 $\pm$0.67 & 5.45 $\pm$0.67 &5.24 $\pm$0.76 & 5.02 $\pm$0.63& 5.45 $\pm$0.67 & 5.45 $\pm$0.67 &5.45 $\pm$0.67 \\
    Energy &2.30 $\pm$0.04 &1.75 $\pm$0.21 & 5.45 $\pm$0.67 &1.60 $\pm$0.24 & 0.53 $\pm$0.07& 5.45 $\pm$0.67 &5.45 $\pm$0.67 &5.45 $\pm$0.67 \\
    Kin8nm &0.09 $\pm$0.00 &0.08 $\pm$0.00 & 5.45 $\pm$0.67 &0.08 $\pm$0.00 & 0.08 $\pm$0.00 & 5.45 $\pm$0.67 &5.45 $\pm$0.67 &5.45 $\pm$0.67 \\
     Naval &0.00 $\pm$0.00 &0.00 $\pm$0.00&5.45 $\pm$0.67 &0.00 $\pm$0.00 & 0.00 $\pm$0.00 & 5.45 $\pm$0.67 &5.45 $\pm$0.67 &5.45 $\pm$0.67 \\
     Power &4.10 $\pm$0.03 &3.98 $\pm$0.09&5.45 $\pm$0.67 &4.08 $\pm$0.08 & 4.05 $\pm$0.08 & 5.45 $\pm$0.67 &5.45 $\pm$0.67 &5.45 $\pm$0.67 \\
     Wine &0.65 $\pm$0.01 &0.63 $\pm$0.04 & 5.45 $\pm$0.67 &0.63 $\pm$0.04 & 0.63 $\pm$0.04 & 5.45 $\pm$0.67 &5.45 $\pm$0.67 &5.45 $\pm$0.67 \\
     Yacht &1.00 $\pm$0.08 &0.95 $\pm$0.39 & 5.45 $\pm$0.67 &1.45 $\pm$0.51 & 0.77 $\pm$0.31 & 5.45 $\pm$0.67 &5.45 $\pm$0.67 &5.45 $\pm$0.67 \\
     Protein &4.98 $\pm$0.02 & 4.44$\pm$0.08 & 5.45 $\pm$0.67 &4.34 $\pm$0.07 & 4.29 $\pm$0.07 & 5.45 $\pm$0.67 &5.45 $\pm$0.67 &5.45 $\pm$0.67 \\
    \hline
    \\
\end{tabular}

    \caption{Comparison of DeepEns and DVN. PICP improvements are not shown for $> 95\%$ and MPIW improvements are only presented when PICP is atleast $95\%$.}
    \label{tab:deepEns_dvn}
\egroup
\end{table}


\begin{table}[h!]
\bgroup
\def\arraystretch{1.2}
\setlength{\tabcolsep}{5pt}
    \centering
    \begin{tabular}{c c c c c c c c c c}
    \hline
     & \multicolumn{3}{c}{RMSE} & \multicolumn{3}{c}{PICP} &\multicolumn{3}{c}{MPIW}\\
     & DeepEns & DVN  & \% & DeepEns & DVN  & \% & DeepEns & DVN & \%\\
     \hline
    Boston & 3.38 $\pm$ 0.26 & 3.13 $\pm$ 1.02 & -22 &3.06 $\pm$ 1.08 & 2.87 $\pm$ 0.68 & 22 & 3.06 $\pm$ 1.08 &3.06 $\pm$ 1.08 &22\\
    Concrete &5.76 $\pm$ 0.10 &5.45 $\pm$ 0.67 &&5.24 $\pm$ 0.76 & 5.02 $\pm$ 0.63&& 5.45 $\pm$ 0.67 &5.45 $\pm$ 0.67 &\\
    Energy &2.30 $\pm$ 0.04 &1.75 $\pm$ 0.21 &&1.60 $\pm$ 0.24 & 0.53 $\pm$ 0.07&&5.45 $\pm$ 0.67 &5.45 $\pm$ 0.67 & \\
    Kin8nm &0.09 $\pm$ 0.00 &0.08 $\pm$ 0.00 &&0.08 $\pm$ 0.00 & 0.08 $\pm$ 0.00 &&5.45 $\pm$ 0.67 &5.45 $\pm$ 0.67 &\\
     Naval &0.00 $\pm$ 0.00 &0.00 $\pm$ 0.00& &0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 &&5.45 $\pm$ 0.67 &5.45 $\pm$ 0.67 &\\
     Power &4.10 $\pm$ 0.03 &3.98 $\pm$ 0.09& &4.08 $\pm$ 0.08 & 4.05 $\pm$ 0.08 &&5.45 $\pm$ 0.67 &5.45 $\pm$ 0.67 &\\
     Wine &0.65 $\pm$ 0.01 &0.63 $\pm$ 0.04 &&0.63 $\pm$ 0.04 & 0.63 $\pm$ 0.04 &&5.45 $\pm$ 0.67 &5.45 $\pm$ 0.67 &\\
     Yacht &1.00 $\pm$ 0.08 &0.95 $\pm$ 0.39 &&1.45 $\pm$ 0.51 & 0.77 $\pm$ 0.31 &&5.45 $\pm$ 0.67 &5.45 $\pm$ 0.67 &\\
     Protein &4.98 $\pm$ 0.02 & 4.44$\pm$ 0.08 &&4.34 $\pm$ 0.07 & 4.29 $\pm$ 0.07 &&5.45 $\pm$ 0.67 &5.45 $\pm$ 0.67 &\\
    \hline
    \\
\end{tabular}
    \caption{Comparison of DeepEns and DVN. PICP improvements are not shown for $> 95\%$ and MPIW improvements are only presented when PICP is atleast $95\%$.}
    \label{tab:deepEns_dvn}
\egroup
\end{table}
